Rain: RDMA-assisted In-Network Scheduling for Microsecond-scale Workloads

Modern data center applications increasingly require microsecond-scale service time with strict tail latency requirements, which can hardly be realized with existing in-network task schedulers due to their inherent limitations. Specifically, software-based schedulers struggle to balance throughput and latency, while switch-based designs either lack global coordination, rely on packet recirculation heavily, or only offer limited support for large tasks. In light of these restrictions of the state-of-the-arts (SOTAs), we, in this work, propose Rain, an RDMA-assisted in-network scheduler built atop programmable switches that maintains centralized queues while bounding worker-local queues. Rain introduces a bidirectional on-switch queuing mechanism to buffer and match tasks and worker-issued tokens directly in the switch, avoiding worker-side polling and approximating the optimal behavior of join-bounded-shortest-queue without global aggregation. A switch-driven RDMA engine pre-writes arbitrarily large tasks via one-sided WRITE multicasts, keeping only compact metadata on the switch. Slice-aware scheduling further localizes decisions to more homogeneous queues, reducing dispersion-induced head-of-line blocking. Moreover, our study reveals that real-world systems can diverge from theoretical predictions: shallower worker queues do not always improve tail latency. Leveraging this insight, Rain incorporates an adaptive scheduling strategy to optimize worker queue depths and worker-to-slice mappings at runtime. Evaluations with the real-world application RocksDB show that Rain achieves 1.75x higher throughput than the best-performing SOTA while satisfying the same tail latency requirement.

==> Makefile <==
MAIN = main

CONTENT = $(wildcard content/*.tex)
SOURCES = $(MAIN).tex $(CONTENT) references.bib

all: $(MAIN).pdf

$(MAIN).pdf: $(SOURCES)
	@echo "==> Compiling $(MAIN).tex with pdflatex..."
	pdflatex -interaction=nonstopmode $(MAIN).tex
	@echo "==> Running bibtex (if references.bib exists)..."
	@if [ -f references.bib ]; then bibtex $(MAIN); fi
	@echo "==> Second pdflatex pass..."
	pdflatex -interaction=nonstopmode $(MAIN).tex
	@echo "==> Third pdflatex pass..."
	pdflatex -interaction=nonstopmode $(MAIN).tex
	@echo "Build complete: $(MAIN).pdf"

clean:
	@echo "==> Cleaning intermediate files..."
	rm -f $(MAIN).aux $(MAIN).bbl $(MAIN).blg $(MAIN).log \
	      $(MAIN).out $(MAIN).toc $(MAIN).lof $(MAIN).lot \
	      $(MAIN).fls $(MAIN).fdb_latexmk

distclean: clean
	@echo "==> Removing generated PDF..."
	rm -f $(MAIN).pdf

.PHONY: all clean distclean

